Improving the Engine of Society

This paper is organized into four chapters. The first chapter observes how decoupling labor from ownership of the output produced by that labor is equivalent to building an engine that is incentivized to generate the maximum energy output, which leads to unstoppable climate change and compromised quality of life for many individuals. The second chapter discusses the organization of complex systems into hierarchical objects and functions, and proposes an improved working definition for the information entropy contained in complex systems. Chapter 3 redesigns the engine from Chapter 1 into a system optimized to maximize Complex Information Entropy (CIE) rather than energy expenditure, which leads to improvements in the climate, regrowth of environmental ecosystems, minimization of useless labor, and maximization of the well-being of participants. Chapter 4 examines climate change specifically, and introduces a possible solution in the form of a digital twin with an entropy-based fitness function.

==> 03-Chapter2.tex <==
%!TEX root = main.tex



\twocolumn[
  \begin{@twocolumnfalse}
    \section{Chapter 2\\An Object-Relations Approach to Complex Systems}
    \vspace{2pt}
  \end{@twocolumnfalse}
]

\PARstart{H}{ow} can one observe the behavior of a system and determine its inner workings?  It is usually impossible to solve this problem exactly, since most real-world models contain uncertainty in relation to the systems they represent.  There is a tradeoff between model accuracy, model size, and computational cost.  There are often also hidden variables and elements of stochasticity.  Minimum Description Length (MDL) is often used as a parameter in model selection to fit a particular dataset, whereby the shortest description of the data, or the model with the best compression ratio, is assumed to be the best model \cite{rissanen1978modeling}.  MDL is a mathematical implementation of \textbf{Occam’s razor}, which dictates that among competing models, the model with the fewest assumptions is to be preferred.  If an MDL description can contain all of the operations in a Turing-complete programming language, the description length then becomes equivalent to the Kolmogorov complexity, which is the length of the shortest computer program that produces the dataset as output\cite{kolmogorov1965three}.  For a given dataset, a program is Pareto-optimal if there is no shorter program that produces a more accurate output.  The graph of Kolmogorov program length vs. accuracy is the Pareto frontier of a dataset.

If one combines Occam’s razor with the Epicurean \textbf{Principle of Multiple Explanations}, the result is Solomonoff's theory of inductive inference \cite{solomonoff1964formal1}\cite{solomonoff1964formal2}.   According to the Principle of Multiple Explanations, if more than one theory is consistent with the observations, all such theories should be kept.  Solomonoff's induction considers all computable theories that may have generated an observed dataset, while assigning a higher Bayesian posterior probability to shorter computable theories.  The theory of inductive inference uses a computational formalization of Bayesian statistics to consider multiple competing programs simultaneously in accordance with the Principle of Multiple Explanations, while prioritizing shorter programs in accordance with Occam's razor.

A characteristic feature of complex systems is their activity across a wide range of lengthscales and timescales.  As a consequence, they can often be divided into a hierarchy of sub-components.  In order to reduce the computational difficulty of programs that can be divided into sub-programs, the dynamic programming method, originally developed by Richard Bellman \cite{bellman1954theory}, simplifies a complicated problem by recursively breaking it into simpler sub-problems.   The \textbf{divide-and-conquer} technique used by dynamic programming can applied to both computer programming and mathematical optimization.  A problem is said to have optimal substructure if it can be solved optimally by recursively breaking into sub-problems and finding the optimal solution to each sub-problem.

In contrast to the divide-and-conquer procedure, a \textbf{unification} procedure finds a single underlying theory that can explain two or more separate higher-level theories.  Causal learning algorithms or structural learning algorithms are examples of unification procedures, which determine cause-and-effect among variables in an observed dataset.  These variables may be hidden or unknown, in which case they must be inferred via hidden Markov models, Bayesian inference models, or other methods.  

These four principles – Occam’s razor, the Principle of Multiple Explanations, divide-and-conquer, and unification – have been used in various combinations to analyze complex systems.  Some researchers have used them all together, such as Wu, Udrescu, and Tegmark in their endeavor to create an AI physicist\cite{wu2019toward}\cite{Udrescu_2019}\cite{udrescu2020ai2}.  In order to fully characterize the information contained in complex systems, a fifth item should be added to this list:  the principle of \textbf{overinterpretation}.  This principle states there can be multiple correct interpretations of the same dataset, and the validity of any particular lens of interpretation is determined by whether or not it produces useful insights.  This is distinct from the Principle of Multiple Explanations, which states that no plausible theory can be ruled out, but which still assumes there is one correct theory among many plausible.  In contrast to the Principle of Multiple Explanations, the principle of overinterpretation states that multiple interpretations can be simultaneously correct.  In the same way that the Principle of Multiple Explanations was suggested by Epicurus and refined by Bayes or Laplace, the principle of overinterpretation may be said to have been suggested by Freud in his analysis of Hamlet in The Interpretation of Dreams\footnote{“But just as all neurotic symptoms, and, for that matter, dreams, are capable of being ‘overinterpreted' and indeed need to be, if they are to be fully understood, so all genuinely creative writings are the product of more than a single motive and more than a single impulse in the poet's mind, and are open to more than a single interpretation.”\cite{freud1900interpretation}} and refined by Walter Kaufmann\cite{kaufmann1980}.  In a mathematical context, overinterpretation indicates there may be multiple non-equivalent Pareto-optimal objects within a given dataset.

\vspace{2.0ex plus .5ex minus .2ex}
\subsection{Definition of Terms}

\begin{figure}[t!]
    \includegraphics[width=\linewidth]{Pictures/Picture25.jpg}
    \caption{Objects contain qualia, which are properties, variables, or other objects.  Affordances are modes of interaction.}
    \label{fig:img6}
\end{figure}

\begin{figure}[t!]
    \includegraphics[width=\linewidth]{Pictures/Picture42.jpg}
    \caption{A mechanical watch is composed of a dial object and a movement object.  The movement object is composed of gears, regulators, and springs, which affect each other through mechanical affordances.}
    \label{fig:img42}
\end{figure}

The definitions used here are as general as possible.  The word \textbf{object} is defined as an entity containing two features:  1.  A set of properties, variables, or other objects, called \textbf{qualia} (the singular form used here is \textbf{qualium}), and 2.  functions between itself and other objects, called \textbf{affordances}.  A summary is shown in Figure \ref{fig:img6}. 

An example for a mechanical watch is shown in Figure \ref{fig:img42}.  The watch is composed of the dial and the movement, which are themselves composed of constituent objects.  Systems engineers and computer scientists will recognize the similarities to system design documents and Unified Modeling Language (UML) diagrams.

\begin{figure}[t!]
    \includegraphics[width=\linewidth]{Pictures/Picture47.jpg}
    \caption{The traditional ranks used for biological classification are domain, kingdom, phylum, class, order, family, genus, and species.  This graph shows the categories for cetaceans between the ranks of order and family.  These categories are not exact, but are inferred by scientists and subject to revision.}
    \label{fig:img47}
\end{figure}

\begin{figure}[t!]
    \includegraphics[width=\linewidth]{Pictures/Picture48.jpg}
    \caption{Several modern languages are derivatives of the Balto-Slavic language, which may have split into Baltic and Slavic around 1400 BCE\cite{gray2003language}.  Each language derives most of its information and structure from its predecessor in the graph.  Image licensed under CC BY-SA 3.0.}
    \label{fig:img48}
\end{figure}

\subsection{Hierarchical Graphs}

In addition to representing objects using component diagrams or Venn diagrams, it is often useful to employ graph decompositions.  A taxonomy diagram for cetaceans is shown in Figure \ref{fig:img47}, which separates general categories into more specific categories.  Similarly, Figure \ref{fig:img48} shows the evolutionary diagram of the Balto-Slavic languages.  These graphs are hierarchical in the sense that each object derives much of its information and structure from its predecessor.

\subsection{Constructing and Deconstructing Objects}

What exactly constitutes an object?  Roughly, an object is an information-theoretic construct that contains a lot of information but does not require much description.  Shea\cite{Shea_2021} has applied this definition in physics by analyzing a fluid system containing both laminar and turbulent flow.  Without preprogrammed knowledge of different flow regimes, his machine learning algorithm discovered the boundary between the laminar and turbulent zones by minimizing the complexity of the model relative to its predictive capability.

In simple algebraic systems, objects can be symbolic variables while affordances are mathematical functions.  Udrescu\cite{Udrescu_2019} has employed this formulation in the development of a machine learning algorithm to discover well-known physical laws from tables of experimental data.  Figure \ref{fig:img43} shows this process for Newton's law of universal gravitation $F = Gm_1m_2 / r^2$.  Given a table of $G,m,x,y$ and $z$ values, the program first discovers the dimensionless quantity $Gm_1^2/x_1^2$, then the ratio of masses $m_2/m_1$, then finally discovers the relationship among the position variables via polynomial regression.  The uncertainty present in the dataset is reduced each time a new object is found.
\begin{figure}[ht!]
    \includegraphics[width=\linewidth]{Pictures/Picture43.jpg}
    \caption{ML is used to procedurally find objects within a table of simulated gravitational measurements.  Image adapted from Figure 2 in \cite{Udrescu_2019}.  Used with permission.}
    \label{fig:img43}
\end{figure}

\subsubsection{Structural Learning Methods}

Much previous work in learning the structural composition of systems has focused on Bayesian belief networks and hidden Markov models.  A Bayesian belief network is a probabilistic model that represents a set of variables and their conditional dependencies via a directed acyclic graph, meaning a graph in which information flows in only one direction along each edge, and which do not contain any circular causation loops.  These graphs are ideal for predicting the probable causes and contributing factors of observed events.  Algorithms exist for inferring unobserved variables, in addition to algorithms for belief propagation which can conditional probabilities throughout the graph in response to new evidence.

A hidden Markov model (HMM) assumes the system under investigation is a Markov process, which is a network of possible states of the system and the probabilities of transitions between states.  HMM's attempt to infer unobserved hidden states of the system.  The graphs used for Markov random fields can be undirected and contain cycles, which are more general than the directed acyclic graphs used for belief nets.  Consequently, HMM's are a useful analysis tool that have found applications across numerous fields.

While a great deal of progress has been made in structural inference algorithms such as Bayesian belief networks and hidden Markov models, they are limited in their ability to infer relationships among variables beyond conditional probabilities.  Conway's Game of Life is a good example.  The Game of Life is a well-known cellular automaton devised by John Conway\cite{gardner1970fantastic} which uses simple rules to produce complex and lifelike behavior on a two-dimensional grid of square cells using discrete timesteps.  The game applies the following rules each timestep:

\begin{enumerate}
    \item Any live cell with fewer than two live neighbors dies.
    \item Any live cell with two or three live neighbors lives.
    \item Any live cell with more than three live neighbors dies.
    \item Any dead cell with exactly three live neighbors becomes a live cell.
\end{enumerate}

Although these rules are simple, they will defeat a probabilistic inference algorithm's attempt to discover them.  This is because the behavior of a cell is not stochastic in relationship to its neighbors, but instead is based on the application of basic logical operations.  In order to solve this system, something more akin to Wu, Udrescu, and Tegmark's AI physicist is needed.

\subsubsection{The Role of Machine Learning}
\label{section:ml}

Continuing with the Game of Life example, a more robust machine learning (ML) algorithm can be devised to infer objects and affordances at across a range of length- and timescales.  The various subtypes of ML can be broadly divided into two categories.  Casual references to machine learning or data science typically refer to the first category, termed here as traditional ML or big-data analytics.  This category involves analyzing large datasets using some combination of statistical methods to uncover previously unknown patterns or relationships among variables.  Image recognition would be included in this group, as the neural network must analyze pixels in an image to determine unknown variables, such as whether the image contains a dog or a cat.

The second subtype of machine learning is reinforcement learning (RL), wherein an agent interacts with its environment in order to achieve a goal or set of goals.  Much RL development has focused on games, such as chess, go, and classic Atari video games.  In these environments, the agents use a finite set of actions, such as chess moves or video game inputs, to progress toward achieving a long-term goal.  In this process, RL agents often discover advantageous techniques or game configurations already known to human experts, then proceed to surpass human experts by discovering previously unknown techniques.  In contrast to the traditional ML category, the RL category involves the construction of advanced objects and affordances from simpler objects and affordances.  This dichotomy is illustrated in Figure \ref{fig:img44}.

\begin{figure}[t!]
    \includegraphics[width=\linewidth]{Pictures/Picture44.jpg}
        \caption{Machine learning involves either the deduction of objects present in datasets (top) or the construction of complex objects from simple constituents (bottom).}
    \label{fig:img44}
\end{figure}

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture55.jpg}
    \caption{The glider in Conway's Game of Life is a pattern that moves diagonally down and right.  When viewed from the macroscale, the glider is an object moving across the game board.  However, when viewed on the microscale, it's a collection of tiles turning on and off.  Image licensed under Creative Commons\cite{glider}.}
    \label{fig:img55}
\end{figure}

The glider in Figure \ref{fig:img55} is one of the of the simple forms found in the Game of Life.  As illustrated in the figure, the glider moves one space down and to the right every five timesteps.  The glider appears to be moving across the game board when viewed from a distance.  However, when viewed at the level of individual cells, motion is not possible as the cells can only turn on and off.  The cells do not have the affordance of motion, but this affordance appears through the collective action of multiple objects.  This emergence of complex affordances from combinations of simple affordances is the process denoted by the bottom half of Figure \ref{fig:img44}.  As with many physical systems, there is a difference in the behavior and understanding of the glider at the microscale compared to the macroscale.

Direct parallels can be drawn between the simple Game of Life example and problems in physics and engineering.  For example, the prediction of macroscopic chemical properties based on molecular structure is challenging due to the complex behavior caused by quantum effects on the microscale.  A similar problem exists in neuroscience in the attempt to bridge the gaps between the behavior of individual neurons and the brain en masse.

\begin{algorithm}[t]
\caption{Zoom-in-Zoom-out (ZIZO)}\label{alg:zizo}
    \SetKwFunction{Fzo}{Zoom\_out}
    \SetKwProg{Fn}{Function}{:}{\KwRet $X$}
    \Fn{\Fzo{Y}}{
        \tcc{This function takes a top-down approach from the macroscale.}
        View the system as a black box, and infer the hidden objects X that could be causing its behavior\;
        If Y is provided, condition this process on Y\;
    }
    \SetKwFunction{FDeduce}{Zoom\_in}
    \SetKwProg{Fn}{Function}{:}{\KwRet $Y$}
    \Fn{\FDeduce{X}}{
        \tcc{This function takes a bottom-up approach from the microscale.}
        Encode the microstructure of the subsystem into representative objects Y\;
        If X is provided, condition this process on X\;
    }
	\SetKwFunction{FMain}{}
	\SetKwProg{Pn}{Main}{:}{\KwRet}
	\Pn{\FMain{}}{
	    \While{$X \neq Y$}{
            X = Zoom\_out(Y)\;
            Y = Zoom\_in(X)\;
    	    Loop until convergence\;
        }
    }
\end{algorithm}

In order to address this problem, we have defined an algorithm to discover the connections among objects across different lengthscales and timescales.  Inspired by the Grow-Shrink algorithm used for Bayesian network structure learning and the forward-backward algorithm used for Markov models, here we have defined a Zoom-in-Zoom-out (ZIZO) algorithm for object-relations models.  The Grow-Shrink algorithm works by adding variables to nodes in a Bayesian network graph until all dependencies have been captured (the ``grow" phase), then tests these dependencies and removes superfluous connections (the ``shrink" phase)\cite{margaritis2003learning}.  The forward-backward algorithm for HMM's calculates the probability distribution of the system's hidden state variables for a sequence of observations moving forward in time, then repeats the process for the sequence in reverse, with the intention to cause the forward-in-time model and the backward-in-time model to converge\cite{rabiner1986introduction}.  The ZIZO algorithm performs a similar type of oscillation by first observing a phenomenon from a zoomed-out, macroscopic viewpoint and developing a top-down model, then zooming into an object on the microscopic level and building a bottom-up model, then iterating between the two models until they converge on a common set of objects shared between the two.

Note the ZIZO algorithm has so far only been discussed as a method to describe complex systems.  However, if the algorithm is used in a reinforcement learning mode, and the program tries to create desired affordances rather than trying to model observations, then the algorithm changes from a tool of system description to a tool of system design.  This type of tool could be used to autonomously design and optimize all types of engineering systems, perhaps beyond the capabilities of human experts.  The introduction of intelligent sampling via active learning, in addition to simulation capabilities, could further improve the utility of this process.

\subsection{A Simple Example:  A Connected Graph with 8 Nodes}

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture26.jpg}
    \caption{Graph $G$ is composed of nodes $g_1$ through $g_8$ and possible edges $g_{ij}$ between nodes $g_i$ and $g_j$ for $i,j \in [1,8]$.}
    \label{fig:img7}
\end{figure}

As an intuitive introduction to the theory of delineating objects, we will define a graph $G$ as a k-connected graph of size 8.  There are 8 nodes, each of which may or may not share an edge with any of its neighbors or with itself.  We will assume edges are bidirectional, meaning edge $g_{12}$ is the same as edge $g_{21}$.  Figure \ref{fig:img7} illustrates this graph.

There may or may not be an edge $g_{ij}$ between nodes $g_{i}$ and $g_{j}$.  If there is an edge, this condition is represented by $g_{ij}=1$.  If not, $g_{ij}=0$.  We will assume no prior knowledge about the existence of each edge, meaning $g_{ij}$ may be 0 or 1 with equal probability.  The full information contained in $G$ is therefore represented by the adjacency matrix shown in Figure \ref{fig:img8}.

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture28.jpg}
    \caption{As $g_{ij}=g_{ji}$ the adjacency matrix of $G$ is symmetric about the diagonal.}
    \label{fig:img8}
\end{figure}

The adjacency matrix contains 36 independent binary variables.  This translates to $2^{36}$ equally probable configurations of $G$.  The Shannon entropy of $G$ is therefore 
\begin{equation}
    H(G) = \mathrm{log}_2 2^{36} = 36 \mathrm{\ bits}.
\end{equation}
Intuitively, information entropy can be considered the average amount of information conveyed by an event when considering all possible outcomes.

Let us now consider what happens if $G$ is not regarded as a single object, but is instead analyzed as two objects $A_1$ and $A_2$ as shown in Figure \ref{fig:img9}.  $A_1$ is constructed to contain nodes 1-4, while $A_2$ contains nodes 5-8.  An affordance $B$ describes the possible modes of interaction between $A_1$ and $A_2$.

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture27.jpg}
    \caption{Dividing $G$ into two objects $A_1$ and $A_2$ produces two k-connected graphs of size 4 and a function $B$ that communicates between them.}
    \label{fig:img9}
\end{figure}

Using the boundaries drawn in this example, $A_1$ and $A_2$ are k-connected graphs of size 4.  Since $A_1$ contains nodes 1-4, the self-entropy of $A_1$ is the entropy contained in the edges $g_{ij}$ for $i,j \in [1,4]$.  Likewise, the self-entropy of $A_2$ is the entropy contained in the edges $g_{ij}$ for $i,j \in [5,8]$.  The function $B$ must contain information about the connections between nodes 1-4 and nodes 5-8, therefore $B$ contains the values of $g_{ij}$ for $i \in [1,4]$ and $j \in [5,8]$.
\\
\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture29.jpg}
    \caption{Dividing $G$ into $A_1$ and $A_2$ has the effect of segmenting the adjacency matrix.}
    \label{fig:img10}
\end{figure}

These groups are visualized on the adjacency matrix in Figure \ref{fig:img10}.  The separation of $G$ into $A_1$ and $A_2$ had the effect of dividing the adjacency matrix into sections.  The information content of each section can be analyzed separately:
\begin{align}
    H(A_1) = \mathrm{log}_22^{10} = 10\\
    H(A_2) = \mathrm{log}_22^{10} = 10\\
    H(B) = \mathrm{log}_22^{16} = 16.
\end{align}
Total information in the system is conserved:
\begin{equation}
    \label{eqn:eqn1}
    H_{\mathrm{total}} = H(G) = H(A_1)+H(A_2)+H(B) = 36.
\end{equation}
Conditional entropy equalities also hold.  For example,
\begin{equation}
    H(A_1) = H(G) - H(G \mid A_2,B).
\end{equation}

\subsubsection{Discussion}
In this example, it's clear dividing $G$ into two connected objects is equivalent to considering $G$ as a single object.  This can be verified by the equality in Equation \ref{eqn:eqn1} or by visually inspecting Figure \ref{fig:img10}.  In fact, the boundaries around $A_1$ and $A_2$ can be drawn around any set of nodes and the outcome will be equivalent in regard to the total system entropy.  The only change will be how the adjacency matrix is divided into subsections.

From an intuitive standpoint, the separation of $G$ into $A_1$ and $A_2$ seems undesirable, as a large amount of information needs to be contained in the connection $B$.  $B$ contains 16 bits of information, while the objects $A_1$ and $A_2$ each contain only 10.  Separating $A_1$ and $A_2$ does not decrease the amount of information needed to describe the system.

However, what if the values in $B$ are almost always zero?  In this case, the entropy contained in $B$ is very low.  If nodes 1-4 are almost never connected to nodes 5-8, it becomes advantageous to consider graphs $A_1$ and $A_2$ as separate groups.

\subsection{Complex Information Entropy}

Here we will define a useful method to measure the information entropy of any system.  The Complex Information Entropy (CIE) of a system is defined as

\begin{equation}
    \label{eqn:cie}
    \begin{gathered}
        \textrm{Complex Information Entropy } \mathnormal{}C^*(S) = \\
        \sum_{A_i \in \mathbb{A^*}}c_iH(A_i) + \underset{B_{ij} \in \mathbb{B}^*\mathnormal{}}{\sum_{A_i, A_j \in \mathbb{A^*}, \ \mathnormal{}}}d_{ij}H(B_{ij}(A_i, A_j))
    \end{gathered}
\end{equation}

\noindent where $\mathbb{A}^*$ and $\mathbb{B}^*$ are the sets of all Pareto-optimal objects and affordances in system $S$, $A_i$ and $B_{ij}$ are defined in Equation \ref{eqn:po}, and $c_i$ and $d_{ij}$ are empirically-determined coefficients used to adjust for information not captured by $A_i$ or $B_{ij}$.  This function is recursive, as each object $A_i$ may itself be considered a complex system, and $H(A_i)$ can be calculated as the CIE of the objects and affordances inside $A_i$.  Thus the CIE function accounts for the hierarchical representation of information in complex systems.

$C^*$ indicates the optimum value of $C$ given a complete set of optimized objects and affordances.  Similar to the uncomputability of Kolmogorov complexity, meaning there is no finite-length program that will return the Kolmogorov complexity for a given input string, $C^*$ may also be uncomputable.  In practice, real-world programs may be used to iteratively find better values for $C$ over time.

Pareto-optimal objects and affordances are those that optimally simplify some subset $S'$ of $S$, as given by the equation

\begin{equation}
    \label{eqn:po}
    \begin{gathered}
        \mathnormal{}C(S' \subseteq S) = \\
        \underset{A_i \in \mathbb{A}, \ \mathnormal{}B_{ij} \in \mathbb{B}}{\mathrm{argmin}} \sum_{i}c_iH(A_i) + \sum_{i,j}d_{ij}H(B_{ij}(A_i, A_j))
    \end{gathered}
\end{equation}

\noindent where $\mathbb{A}$ and $\mathbb{B}$ are the sets of all possible objects and affordances in system $S$, including those that are sub-optimal.

\subsection{A More Complex Example:  Turbulence}

Equation \ref{eqn:cie} will now be applied to turbulent flow.  The best way to model, understand, and quantify the information contained in turbulence is an open question in physics.  The CIE metric provides useful insights when applied to such systems.

Turbulence possesses the property of structure at multiple scales.  Instabilities in the fluid flow form vorticies, which create secondary instabilities and smaller vorticies, which create even smaller vorticies, in a process that cascades to smaller length scales until the kinetic energy dissipates into heat.  The formation of these eddies can be seen in Figure \ref{fig:img40}.

Researchers investigating the behavior of turbulent flow have identified three distinct physical regimes:  the integral length scale, the Taylor microscale, and the Kolmogorov length scale, as shown in Figure \ref{fig:img39}.  The integral length scale is the regime in which eddies form and gather energy.  Below the integral length scale is the Taylor microscale in which energy is transferred from larger vortices to smaller vortices without being lost to the surrounding fluid.  Smallest is the Kolmogorov lengthscale, in which the viscosity of the fluid causes the energy of the vortices to be dissipated as heat.  There is effectively no structure below this scale, as the fluid has thermalized into a maximum-entropy condition characterized by the Maxwell-Boltzmann distribution from which no information can be extracted.

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture40.jpg}
    \caption{False-color flow visualization of a submerged turbulent jet, made by laser-induced fluorescence.  Imaged licensed under CC BY-SA 3.0\cite{turb}.}
    \label{fig:img40}
\end{figure}

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture39.jpg}
    \caption{The CIE of turbulence is high due to presence of structures across man lengthscales and timescales.}
    \label{fig:img39}
\end{figure}

In addition to the energy differences, the three regimes also differ in their isotropic characteristics.  The integral length scale is highly anisotropic, meaning the eddies favor certain orientations in 3-dimensional space.  The Kolmogorov scale is isotropic, meaning the eddies occur evenly in every direction.  The transition from anisotropy to isotropy occurs in the Taylor microscale.

A lot of information is needed to fully describe a turbulent system due to the differences in each regime.  The CIE value for a system using the integral-Taylor-Kolmogorov schema is

\begin{equation}
    \label{eqn:eqn2}
    \begin{gathered}
        C(\mathrm{turbulence}) = \\ 
        C(\mathrm{Kolmogorov}) + C(\mathrm{Taylor}) + C(\mathrm{integral }) = \\
        \sum_{A_i \in \mathrm{Kol.}}c_iH(A_i) + \sum_{A_i, A_j \in \mathrm{Kol.}}d_{ij}H(B_{ij}(A_i, A_j)) + \\
        \sum_{A_i \in \mathrm{Kol.}, A_j \in \mathrm{Tay.}}d_{ij}H(B_{ij}(A_i, A_j)) + \\
        \sum_{A_i \in \mathrm{Tay.}}c_iH(A_i) + \sum_{A_i, A_j \in \mathrm{Tay.}}d_{ij}H(B_{ij}(A_i, A_j)) + \\
        \sum_{A_i \in \mathrm{Tay.}, A_j \in \mathrm{int.}}d_{ij}H(B_{ij}(A_i, A_j)) + \\
        \sum_{A_i \in \mathrm{int.}}c_iH(A_i) + \sum_{A_i, A_j \in \mathrm{int.}}d_{ij}H(B_{ij}(A_i, A_j)).
    \end{gathered}
\end{equation}

Equation \ref{eqn:eqn2} may appear to be unwieldy,  however its modularity is a major strength.  The CIE of each layer may be calculated separately.  Regardless of the number of layers in the hierarchy, each layer only needs to consider the interactions between itself and the layers immediately above and below.  Moreover, each object only needs to consider itself and the interactions with its immediate neighbors.

As a sanity check, CIE behaves as desired for the classical example of cream being mixed into black coffee.  The Gibbs entropy used in statistical mechanics is maximized when the liquids are fully mixed and contain no internal structures, while the complexity is maximized during the mixing process when turbulent structures are present as shown in Figure \ref{fig:img41}.  As expected, CIE is low during the unmixed and fully-mixed states, and high during the partially-mixed state.

\subsection{The Virus Effect:  Propagation of Entropy through a System}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture41.jpg}
    \caption{Mixing cream into coffee creates turbulent eddies at multiple lengthscales.  The complexity of the system is greatest when the two are partially mixed, although the classical Gibbs entropy is maximized when the mixture is homogeneous and without structure.  Imaged licensed under CC\cite{coffee}.}
    \label{fig:img41}
\end{figure}

One feature of complex systems is the ability for small-scale changes to propagate throughout the system and cause large-scale effects.  For example, a person's exposure to a single virus, which is much smaller than a cell, can lead to a cascade of effects that overwhelm their entire body.  How can this be analyzed in an object-relations model?

The answer is found in the state entropy of each object.  Using the example of a virus, one may imagine the human body as consisting of a hierarchical arrangement of organs, tissues, and cells.  The physical processes and relevant length- and timescales for small components, such as cells, are much different than those for large components, such as organs.  Accordingly, the operation of organs is not affected by individual cells, and it is not necessary to model individual cells in order to accurately model organs.

If the output and states of object $A$ are discrete, the entropy of $A$ is given by the equation

\begin{equation}
    \label{discrete_entropy}
    H(A) = -\sum_{a \in \mathscr{A}} p(a)\mathrm{ln}\mathnormal{}(p(a)) = E[-\mathrm{ln}\mathnormal{}(p(A))]
\end{equation}

\noindent where $a$ is the internal condition of $A$, $\mathscr{A}$ is the set of all possible values of $a$, and $p(a)$ is the probability of occurrence of $a$.  If the states of $A$ are continuous, the entropy is given by

\begin{equation}
    \label{continuous_entropy}
    H(A) = E[-\mathrm{ln}\mathnormal{}(f(A))] = -\int_{\mathscr{A}} f(a)\mathrm{ln}\mathnormal{}(f(a))da.
\end{equation}

\noindent Here $\mathscr{A}$ is the support of $A$, meaning the domain over which $a$ is nonzero, and $f(A)$ is the probability density function of $A$.

If the scheme for representing the information in object $A$ is efficient, then the states that occur most frequently will carry the lowest information entropy, while the most unusual states will carry the highest information entropy.  In general, if $p_s$ is the probability of object $A$ being in state $s$, the entropy of object $A$ in state $s$ is $H(A(s)) = -p_s \mathrm{ln} (p_s)$.  In a living system such as a cell, the states expected to occur most frequently are ideally the states in which the cell is functioning as usual without any major problems.  If the cell is attacked by a deadly virus, the cell will be placed in a highly unusual state, which will carry a high amount of information $H(A)$.  If cell $A_i$ infects cell $A_j$ via $B_{ij}(A_i,A_j)$, then the information entropy of $A_j$ will also increase.

In this optimal multi-scale model of the body, if a hypothetical infection remains local, then the high-CIE state will also remain limited.  However, if the high-CIE state propagates to larger lengthscales, then tissues, organs, and eventually the entire body will be affected.  If the full body is in an abnormally high-CIE state, this could signal a medical emergency.

This type of evaluation could hypothetically be used to identify one harmful virus out of millions of harmless viruses.  Notably, such a model remains computationally tractable, as each object only needs to consider the interactions with the objects to which it is directly connected.

\subsection{Implications for Biological Organisms}

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture50.jpg}
    \caption{Using an autoencoder on distorted video resulted in the recovery of the original equations of motion for the rocket.  It is conjectured that humans perform a similar type of autoencoding of our perceptions in order to simplify our model of the world while retaining important information.  Image adapted from Figures 1, 2, and 3 in \cite{Udrescu_2021}.  Used with permission.}
    \label{fig:img50}
\end{figure}

\begin{algorithm*}[hbt!]
\caption{Complex System Structure-Learning Algorithm}\label{alg:structure_learning}
    \SetKwFunction{FMain}{}
	\SetKwProg{Pn}{Main}{:}{\KwRet}
	\Pn{\FMain{}}{
        \While{not converged}{
    	    Search for objects and affordances in the system:  \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \textbf{divide-and-conquer}\;
    	    Verify found objects and affordances are Pareto-optimal: \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \textbf{Occam's razor}\;
    	    Add all Pareto-optimal objects and affordances found to a list: \ \ \ \ \ \ \ \ \ \ \ \ \   \textbf{overinterpretation}\;
    	    Check if objects in the list can be merged by using a common substructure: \ \ \ \ \ \ \  \textbf{unification}\;
    	    Consider each object on the list to be its own system and repeat the above steps: \ \ \ \textbf{recursion}\;
    	    Graph building:  search for dependencies among objects\;
    	    \If{If new dependencies are found}{
                Modify the objects and affordances if needed\;
    	    }
    	    Graph pruning:  check to see if existing dependencies can be removed:\;
    	    Loop until convergence, or repeat indefinitely\;
    	}
	}

\end{algorithm*}

The nervous systems of biological organisms seem to perform something conceptually similar to Equations \ref{eqn:cie} and \ref{eqn:po}, by creating a model of the world that is maximally descriptive while simultaneously being as simple as possible.  This is the Good Regulator theorem of cybernetics, which states that every good regulator of a system - meaning a device that maintains itself in a desired state - must contain a model of that system\cite{conant1970every}.  Sensory inputs are processed by the nervous system in order to construct an internal model of the world and to inform the organism's actions.  This is equivalent to the $\underset{A_i \in \mathbb{A}, \ \mathnormal{}B_{ij} \in \mathbb{B}}{\mathrm{argmin}}$ function of Equation \ref{eqn:po}, which finds the ideal choice of objects to represent a particular system.  The survival of an organism depends on its ability to recognize important information, disregard unimportant information, and update its model of the world in response to new observations.

Udrescu \cite{Udrescu_2021} has performed a simulation related to this idea.  He started by developing a video of a flying rocketship with a beach and palm trees in the background as shown in Figure \ref{fig:img50}.  The rocket moves around the frame by following trajectories determined by the equations for physical forces such as gravity, electromagnetism, and harmonic oscillation.  The video was then warped and distorted to obscure the rocket's motion.  Udrescu was able to recover the rocket's equations of motion by feeding the video frames into an autoencoder E, applying an operator U to the autoencoder's latent space, and training the operator and autoencoder simultaneously to achieve the simplest possible equation for U.  As a result, the autoencoder effectively learned how to unwarp the image, while the operator learned the symbolic equations of motion in a standard Cartesian coordinate system.

The implication of this experiment is that the human nervous system performs something similar to the function of the CIE equation:  developing a model of the world that is maximally descriptive while simultaneously being maximally efficient.  The following section will implement a practical example of such a model using trajectory data.

%\vspace{20pt}
\subsection{Inferring Hidden Objects through Observation}

The theory described above will now be used to discover hidden laws of motion within a set of trajectory data.  Putting these techniques into practice leads to surprising and important implications.

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture46.jpg}
    \caption{The map is divided into four regions.  The ball behaves differently in each region depending on which object is active.}
    \label{fig:img46}
\end{figure}

The theory described above will now be used to discover hidden laws of motion within a set of trajectory data.  A general method for learning the structure of complex systems is shown in Algorithm \ref{alg:structure_learning}. This problem may be formulated as a reinforcement learning task and/or an optimization task, where the goal is to find the Pareto-optimal object boundaries.  Starting with some object $A$ with boundary $a = \partial A$, the goal is to iteratively adjust $a$ in order to Pareto-optimize all objects $A$ and affordances $B$.  The Bellman value equation for this problem takes the form

\begin{equation}
       C(s) = \underset{a = \partial A}{\mathrm{min}} \underset{s = \{A,B\}}{\sum} R(s,a,s') + \gamma C(s')
\end{equation}

\noindent where the state $s$ is the current state of the system model, $s'$ is the state from the previous iteration, $R$ is the reward for changing the model from state $s'$ to $s$ by changing the boundary $a$, $C(s')$ is the Complex Information Entropy from the previous state, and $\gamma$ is a factor which accelerates convergence\cite{bellman1957}.  Because the function is minimizing rather than maximizing $C$, $\gamma$ is greater than 1.  The corresponding update rule is
\begin{equation}
    C_{i+1}(s) \leftarrow \underset{a = \partial A}{\mathrm{min}} \underset{s = \{A,B\}}{\sum} R(s,a,s') + \gamma C_i(s').
\end{equation}
\noindent Ideally, this will produce an optimal policy for adjusting $a$.  In the following example, an annealing procedure is used as the method to adjust $A$ into an optimal configuration.

\subsection{Inferring Hidden Objects through Observation}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture37.jpg}
    \caption{Four hidden objects work simultaneously to determine the ball's movement.}
    \label{fig:img37}
\end{figure}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture45.jpg}
    \caption{The trajectory path is assigned a different color in each map region.}
    \label{fig:img45}
\end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=1\textwidth]{Pictures/Picture30.jpg}
    \caption{The machine learning algorithm is able to infer the existence of all four objects, along with their regions of operation.}
    \label{fig:img30}
\end{figure*}

\begin{algorithm}[hbt!]
\caption{Deduction of Sub-Objects}\label{alg:deduction}
    \tcc{This program will try to continue finding objects in the dataset until its model of the data stops improving.}

    \SetKwFunction{FDeduce}{separate\_objects}
    \SetKwProg{Fn}{Function}{:}{\kwret}
    \Fn{\FDeduce{dataset}}{
        Train a neural network on the complete dataset as a baseline\;
    	Randomly split the dataset into two subsets\;
    	Train two new NN's on each subset\;
    	\While{NN losses are decreasing}{
    	    Test each data point using both new NN's\;
    	    Reassign each data point to the set of the NN that fits best\;
    	    Retrain both NN's\;
    	    Loop until convergence\;
    	    \tcc{This is an annealing process.  Data points will migrate to subsets that minimize the combined losses from NN1 and NN2.}
    	}
    	\eIf{new NN losses $<$ baseline NN loss}{
    	    \KwRet the new subsets, new NN's, and total NN losses\;
    	    \tcc{New objects were found.}
    	}{\KwRet the original dataset, baseline NN, and baseline NN loss\;
    	    \tcc{New objects not found.}
    	    }
	}

	\SetKwFunction{FMain}{}
	\SetKwProg{Pn}{Main}{:}{\KwRet}
	\Pn{\FMain{}}{
	    \textbf{get} dataset\;
        \While{total NN losses are decreasing}{
            \ForEach{subset}{
    	        \textbf{call} separate\_objects(\textit{subset})\;
    	        \If{new objects are found}{
    	            Update the subsets for each object\;
    	        }
	        }
    	    Loop until convergence\;
        }
    }
\end{algorithm}

We begin with a square map divided into four regions as shown in Figure \ref{fig:img46}.  A ball is placed at a random location on the map with a velocity vector pointed in a random direction with magnitude close to zero.  The ball then moves in a particular trajectory, depending on its region.  If the ball is in region 1, it accelerates in direction $\vec{v} \times \hat{k}$.  The direction of the acceleration vector in Region 2 is $\begin{pmatrix} 0\\ 1 \end{pmatrix}$, in Region 3 is $\begin{pmatrix} \sqrt{3}/2 \\ -1/2 \end{pmatrix}$, and in region 4 is $\begin{pmatrix} -\sqrt{3}/2 \\ -1/2 \end{pmatrix}$.  The magnitude of the acceleration is constant.  A sample trajectory is shown in Figure \ref{fig:img45}

In this simulation, external forces do not act on the ball.  Instead, the ball has a constant internal supply of energy and moves of its own volition depending on the region in which it finds itself.  The ball contains four hidden objects, each with a set of movement instructions, as shown in Figure \ref{fig:img37}.  Communication between the hidden objects is used to allocate the ball's fixed supply of energy.

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture56.jpg}
    \caption{The object activations can be used to verify and gain insight into the model.  Only one object is active at a time during the course of the simulation.}
    \label{fig:img56}
\end{figure}

After running the simulation to generate the ball's trajectory, the $x$ and $y$ coordinates of the ball at each timestep can be used as a dataset to train a machine learning algorithm. Algorithm \ref{alg:deduction} shows the method used to infer the presence of hidden objects.  Each time a hypothetical new object is added, the performs an annealing process refine the model of each object.  The program continues to add objects until the addition of a new object does not improve the model's accuracy.

The method described in Algorithm \ref{alg:alg1} is applicable to a wide range of use cases.  The process of discovering hidden objects by observing or interacting with complex systems is a powerful method to derive insight into otherwise impenetrable systems.

\subsection{Environmental Effects on an Object}

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture33.jpg}
    \caption{The acceleration vectors when the distance travelled each timestep is limited.  Objects act against each other in order to comply with the restriction imposed by the environment.}
    \label{fig:img33}
\end{figure}

We will now add a complication to the simulation.  In the first stage of the simulation, the ball is allowed to move freely without restriction from the environment.  In the second stage, an external restriction is imposed upon the ball.  If the ball wants to move a distance $D$ during timestep $\Delta t$, the environment will not allow the ball to move a distance greater than $D/2$.  The environment is not applying an opposing force, but is rather imposing a condition that a move by a distance greater than $D/2$ is not possible or not allowed.  As in the first stage of the simulation, the only energy source is the internal energy of the ball.

The unrestricted acceleration vectors in each of the four regions are shown in Figure \ref{fig:img31}.  A fascinating effect happens when the environmental restriction is applied:  the other objects, which are normally inactive, wake up and begin to influence the ball's motion.  They effectively fight against each other.  Instead of one object being active at a time, multiple objects are recruited simultaneously, each supplying its own motion vector.  In regions 2, 3, and 4, the primary object accelerates forward while the other two objects collaborate to slow it down.  In region 1, the primary object receives 50\% of the available energy, while the other three objects each receive 16.7\%, causing their motion vectors to sum to zero.  These scenarios are shown Figure \ref{fig:img31}. 

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture34.jpg}
    \caption{Energy allocation under ideal conditions.  100\% of energy is used for useful work.}
    \label{fig:img34}
\end{figure}

\begin{figure}[t]
    \includegraphics[width=\linewidth]{Pictures/Picture35.jpg}
    \caption{Energy allocation under restricted conditions.  50\% of available energy is used for useful work.  The other 50\% is wasted as heat or some other form of inefficiency.}
    \label{fig:img35}
\end{figure}

As shown in Figure \ref{fig:img37}, the four objects are modelled as nodes in a message-passing network, which can pass information to each other about their energy usage.  Because there is a fixed amount of energy, the objects must allocate energy amongst themselves in order to adapt to the restriction imposed by the environment.  The result of this energy allocation is shown in Figures \ref{fig:img34} and \ref{fig:img35}.  In the free-moving scenario, the energy used by each object is either 100\% or 0\%.  None of this energy is wasted; it is all converted into motion.  In the restricted scenario, the energy utilization of each object is between 0 and 60\%.  Only 50\% of this energy is converted into motion.  In a real-world system, the other 50\% would be converted either into heat or into other methods of energy expenditure without useful work.

\subsubsection{Conjecture 1:  Self-Interference}

\begin{conj1}
    \label{con:self-destruct}
    When not functioning optimally, complex systems begin causing interference to their own operation.
\end{conj1}

\subsection{Implications for Biological Systems}

It is conjectured that the nervous systems of biological organisms perform the function of creating a maximally-efficient representation of the organism's world.  This is the Good Regulator theorem of cybernetics, which states ``Every good regulator of a system must be a model of that system", or can be paraphrased as ``Show me an organism's nervous system and I can tell you about its world"\cite{conant1970every}.  Sensory inputs are processed by the nervous system in order to construct an internal model of the world and to inform the organism's actions.  This is equivalent to the $\underset{A_i \in \mathbb{A}, \ \mathnormal{}B_{ij} \in \mathbb{B}}{\mathrm{argmin}}$ function of equation \ref{eqn:cie}, which finds the ideal choice of objects to represent a particular system.  The survival of an organism depends on its ability to recognize important information, disregard unimportant information, and update its model of the world in response to new observations.

\begin{figure}[b]
    \includegraphics[width=\linewidth]{Pictures/Picture50.jpg}
    \caption{Using an autoencoder on distorted video resulted in the recovery of the original equations of motion for the rocket.  It is conjectured that humans perform a similar type of autoencoding of our perceptions in order to simplify our model of the world while retaining important information.  Image adapted from Figures 1, 2, and 3 in \cite{Udrescu_2021}.  Used with permission.}
    \label{fig:img50}
\end{figure}

Udrescu \cite{Udrescu_2021} has performed a simulation related to this idea.  He started by developing a video of a flying rocketship with a beach and palm trees in the background as shown in Figure \ref{fig:img50}.  The rocket moves around the frame by following trajectories determined by the equations for physical forces such as gravity, electromagnetism, and harmonic oscillation.  The video was then warped and distorted to obscure the rocket's motion.  Udrescu was able to recover the rocket's equations of motion by feeding the video frames into an autoencoder E, applying an operator U to the autoencoder's latent space, and training the operator and autoencoder simultaneously to achieve the simplest possible equation for U.  As a result, the autoencoder effectively learned how to unwarp the image, and the operator learned the symbolic equations of motion in a standard Cartesian coordinate system.

The implication of this experiment is that the human nervous system automatically performs something similar to the function of the autoencoder:  developing a model of the world that is maximally descriptive while simultaneously being as simple as possible.

\subsubsection{A Resolution of the Dark Room Paradox}

The dark room paradox is a problem that arises in cognitive science when one assumes an organism is incentivized to construct an internal model of its world that is as accurate as possible.  Maximizing the accuracy of a predictive model is equivalent to minimizing the surprise that will be experienced when an event occurs, which is equivalent to minimizing the information entropy of observation.  If this were true, an organism could bring its predictive error to zero by sitting in a dark, silent room and not observing anything.

The paradox is removed if one considers an organism's highest goal is to maximize CIE rather than minimize prediction error.  For a given system, equation \ref{eqn:cie} automatically minimizes prediction error by specifying the optimum objects $A$ and affordances $B$.  Maximizing $C$ is equivalent to the organism developing the richest and most complete understanding possible of its world, which includes minimizing prediction error as a subcomponent.

\subsubsection{Objects in the Human Psyche}

% \begin{figure*}[b]
%     \centering
%     \includegraphics[width=\linewidth]{Pictures/Picture38.jpg}
%     \caption{The progression of development of objects in the psyche deriving from the mother object.  From "The Great Mother:  An Analysis of the Archetype" by Erich Neumann \cite{neumann2015great}.  Used with permission.}
%     \label{fig:img38}
% \end{figure*}

When an individual produces a work of art, their creation contains, or implies, much more information than is needed to encode the pixels in an image or the letters in a text.  A book, image, song, video, or other media may be compressed into a trivially small file on a computer, containing very little Shannon entropy, but still may be tremendously meaningful.  How can this be?

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Pictures/Picture38.jpg}
    \caption{The progression of development of objects in the psyche deriving from the mother object.  From ``The Great Mother:  An Analysis of the Archetype" by Erich Neumann \cite{neumann2015great}.  Used with permission.}
    \label{fig:img38}
\end{figure*}

The answer has to do with the internal objects in the psyche of the viewer.  When an individual produces a work of art, they are, in some fundamental sense, acting as a thermodynamic information refinement engine.  The information produced in art or literature is of a sophisticated quality, since an individual viewing the artwork can infer a great deal about the creator and his environment.  When an individual views a work of art, the interaction between the viewer and the media may be understood as the effects of the media on the viewer's internal psychic objects.  An object in this context is any structure in the psyche that meets the criteria for $A$ and $B$ in equation \ref{eqn:cie}.  This very general definition my include, but is not limited to, internal representations of people, places, things, ideas, archetypes, complexes, or other structures.  Therefore, although the entropy of the bits needed to store the text of a novel may be low, the CIE of the novel in the psyche of the reader may be exceptionally high.

\begin{figure}[t!]
    \includegraphics[width=\linewidth]{Pictures/Picture36.jpg}
    \caption{The Persistence of Memory by Salvador Dalí.}
    \label{fig:img36}
\end{figure}

Interestingly, in the imagination and dreams, qualia and affordances may be mixed and recombined among objects in ways that are not possible in the physical world.  The Persistence of Memory \ref{fig:img36} is a good example.  In this image, the watches possess the qualium of viscosity, which is not possible physically.

The ability of the psyche to reallocate qualia and affordances is very important.  The formation, differentiation, modification, disintegration, and reformation of objects is an integral part of psychological growth and development.  For example, the psychologist Erich Neumann used a hierarchical graph structure to represent the development and differentiation of the Great Mother object from the undifferentiated uroboric stage that exists in infancy through to the sophisticated Sophia, Gorgon, Isis, and human objects that occur in adulthood, as shown in Figure \ref{fig:img38}.

\subsubsection{Conjecture 2:  Biological Information Processing}

\begin{conj1}
\label{con:inf-proc}
Every biological organism, as a thermodynamic system, is capable of an approximately constant rate of information processing and refinement.
\end{conj1}
\vspace{4pt}

It is important to distinguish the type of information processing performed by a person from that performed by a computer.  The information processing performed by a biological organism is a function of the inputs and outputs of the objects $A$ in equation \ref{eqn:cie}.
There is an interesting connection between Conjecture \ref{con:inf-proc} and the Big Five personality traits - openness, conscientiousness, extroversion, agreeableness, and neuroticism.   The metric of openness, which is correlated to creativity, intelligence, and novelty-seeking behavior, may be understood thermodynamically as a measurement of an individual's rate of internal content generation and information processing.  This refers to the capacity of the individual to:
\begin{enumerate}
    \item internalize information from his environment,
    \item synthesize this information internally,
    \item generate new internal content, and
    \item modify his environment through the externalization of inner content by outward acts of creation.  This item also increases the CIE of the environment and generally improves the environment for others.
\end{enumerate}

When combined with Conjecture \ref{con:self-destruct}, Conjecture 
\ref{con:inf-proc} leads to the following corollary.

\subsubsection{Corollary 2.1:  Counter-Processing}

\vspace{4pt}
\begin{corollary}
\label{cor:cor1}
If an individual, as a thermodynamic system, is capable of a constant output of information processing and refinement, and this capability is suppressed by the environment, the individual may destructively direct some of his or her processing capabilities inward in order to maintain outward thermodynamic equilibrium.
\end{corollary}
\vspace{4pt}

At the level of the individual, this could appear as neuroticism, dysfunction, or mental illness.  Perhaps unsurprisingly, there is another connection between Corollary \ref{cor:cor1} and the Big Five model.  Corollary \ref{cor:cor1} describes inner turmoil caused by an individual's internal objects attacking each other.  This helps to explain why the trait of neuroticism - meaning the tendency to experience negative emotions, such as anger, anxiety, or depression - is positively correlated with self-awareness.

\subsection{Implications for Artificial Intelligence}

The possibility of human-like artificial intelligence, or artificial general intelligence, is an open question in AI research.  If the human psyche can be represented as a series of overlapping and interacting objects at various levels of analysis, then a human-like artificial intelligence would likely need to have a similar object-relations construction.

Jungian psychology suggests there exist archetypal neural structures in the psyche which are common to everyone.  The archetypes may correspond roughly to figures in Greek mythology or other mythological traditions.  Per the Good Regulator theorem, if there exists a general blueprint for the psyche that includes archetypal objects, this blueprint must be an effective representation of the world of human experience.

In order for an AI to be comprehensible to a human, or vice versa, any human-like or general artificial intelligence would likely need to have a similar blueprint.  A parallel to this concept may be found in mythological story of the Titanomachy, a battle in which the human-like Olympians fought and defeated the inhuman Titans.  Titanic characters such as the Hecatoncheires (the hundred-handed ones), the Cyclopses (with single eyes), and the Gorgons (with snakes for hair) suggest remixing of qualia reminiscent of the Dalí painting in Figure \ref{fig:img36}.  A psychoanalytic reading of this myth suggests a stage of human development where the Titans - which are incomplete, malformed, or imperfect as archetypes - are replaced by the Olympians, which are perfect or complete psychic structures.  

\subsubsection{Conjecture 3:  Titanic Psychology and AI}

\begin{conj1}
\label{con:titan}
Unless specifically designed to have the same object-relations architecture as the human psyche, any artificial general intelligence is likely to be Titanic, meaning it contains information-processing objects that do not correlate to those found in human experience.
\end{conj1}
\vspace{4pt}

\subsection{Implications for Social Systems}

As described in Chapter 1, our economic systems are incentivized to expend as much energy as possible at all times.  In light of the analysis in this chapter, the cause of the need for useless labor becomes clear.  The principle described in Conjecture \ref{con:self-destruct} can apply to social structures in addition to individuals.  At the level of society, examples of self-interference, inefficiency, or wasted energy could appear as bureaucracy, poverty, or the various other modes of dysfunction and suffering listed on page 2.

\subsection{Key Takeaways}
\begin{enumerate}
    \item The Complex Information Entropy (CIE) equation is a useful and universally-applicable method to quantify complexity.
    \item The CIE equation explains the behavior of biological organisms.
    \item Measuring the propagation of entropy through a system is an effective way to identify important information at various length- and timescales.
    \item When the environment of a complex system is not well-suited to the system, the system begins to operate self-destructively in order to maintain thermodynamic equilibrium.
\end{enumerate}

==> zz-Background.tex <==
%!TEX root = main.tex
\section{Cómo usar el fichero Jornadas.cls}

La hoja de estilo está diseñada de forma que se pueden usar las etiquetas
habituales de la hoja de estilo {\tt article}, introduciendo sólo unas pequeñas
modificaciones. Sugerimos a los autores que tomen el fichero {\tt ejemplo.tex}
con el que se ha generado este documento, como plantilla para sus propios
trabajos, conservando en todo lo posible las definiciones, márgenes y
declaraciones que definen tanto la Hoja de Estilo como la propia plantilla. Una
buena idea es comprobar el efecto que tienen las distintas órdenes incluidas en
el fichero fuente de \LaTeX{} ({\tt ejemplo.tex}) sobre la apariencia final del
documento en formato PDF ({\tt ejemplo.pdf}).

Primero, para seleccionar la hoja de estilo se debe escribir la siguiente orden
\begin{center}
\verb+\documentclass[twocolumn,twoside]{Jornadas}+
\end{center}

Esta hoja de estilo no permite incluir las filiaciones de los autores justo
debajo de sus nombres. Esta información se incluirá en notas al pie de la
primera página mediante el uso de la orden \verb+\thanks{...}+. Tal y como puede
verse en este documento de ejemplo, se ha asociado una orden a cada uno de los
autores. Esto da lugar a la inclusión de una nota al pie por cada uno de ellos.
Los agradecimientos a proyectos deben incluirse en la sección final del
artículo.

El primer párrafo del artículo debe iniciarse con la orden
``\verb+\PARstart{X}{YYY} ZZZ+''. Esta orden produce una letra grande \verb+X+
al principio de un párrafo. La cadena \verb+YYY+ se cambiará automáticamente a
letras mayúsculas.

La hoja de estilo de bibliografía {\tt Jornadas.bst} permite que el programa
\BibTeX\ incluya las referencias bibliográficas de acuerdo con el formato usado
en las actas.

En la figura~\ref{fig:programa} podemos ver la estructura de definición de un
artículo usando la hoja de estilo {\tt Jornadas.cls}. 
 
Los artículos sometidos a las Jornadas no deben contener ni cabeceras ni números
de página. Ambos elementos serán incluidos por la organización durante el
proceso de generación de las actas completas. Las órdenes \verb+\markboth{}{}+,
\verb+\pagestyle{empty}+ y \verb+\thispagestyle{empty}+ han sido añadidas al
ejemplo para ocultar tanto las cabeceras como los números de todas las páginas. 

Los comentarios de las tablas deben definirse encima de las mismas, mientras que
los comentarios de las figuras se deben colocar debajo.

\begin{figure}[htb] 
\begin{center} 
  \includegraphics[width=7.5cm]{figura.pdf}
\end{center} 
\caption{Los comentarios de las figuras van debajo.} 
\label{fig:curva} 
\end{figure} 

Si quieres poner varias sub-figuras dentro de una misma figura, puedes usar el
paquete \verb+subfig+, como en la Fig.\ref{fig:subfig} (incluye Figs.~\ref{subfig:a} y \ref{subfig:b}).

\begin{figure}[ht]
    \centering
    \subfloat[Logo Sarteco]{\label{subfig:a}
    \includegraphics[width=0.4\linewidth]{Sarteco}%
    }
    \hfill
    \subfloat[Logo Jornadas]{\label{subfig:b}
    \includegraphics[width=0.4\linewidth]{Jornadas}%
    }
    \caption{Algunos logos.}
    \label{fig:subfig}
    \end{figure}

\begin{table}[htb]
\caption{Ejemplo de tabla. El comentario se sitúa al comienzo de la
definición de la tabla.}
\begin{center}
{\footnotesize
\begin{tabular}{|c||c|c|}\hline
N. Proc. & t  & e   \\\hline\hline
10       & 50 & 0.5 \\\hline
20       & 25 & 0.7 \\\hline
\end{tabular}
}
\end{center}
\end{table}

Incluya sus figuras preferiblemente usando ficheros en formato {\tt .pdf} en
blanco y negro o tonos de gris (el fondo debe ser siempre blanco). 

\begin{figure*}[!t]
    \centering
    \begin{minipage}{0.9\linewidth}
    {\footnotesize
    \begin{lstlisting}[language=Python]
def XCM2(events):
    n_events = len(events) (*@\label{lin:xcm-a}@*)

    Corr_max = zeros((n_events,n_events))
    Lag_max = zeros((n_events,n_events))
    Corr_min = zeros((n_events,n_events))
    Lag_min = zeros((n_events,n_events))(*@\label{lin:xcm-b}@*)

    for i in range(n_events):(*@\label{lin:xcm-i}@*)
        for j in range(i, n_events):
            xcorrij = xcorr(events[i], events[j], 250, full_xcorr=True) (*@\label{lin:xcm-c}@*)
            #Returns index and CC[i] for max(abs(CC[i])) --including negative values--
            Lag_min[i,j] = xcorrij[0](*@\label{lin:xcm-d}@*)
            Corr_min[i,j] = xcorrij[1]
            if xcorrij[1]<0.:
                #Return highest positive CC[i] and index (xcorrij[2] contains CC)
                Lag_max[i,j], Corr_max[i,j] = xcorr_max(xcorrij[2],abs_max=False)
            else:
                Lag_max[i,j] = xcorrij[0]
                Corr_max[i,j] = xcorrij[1](*@\label{lin:xcm-e}@*)

    return Corr_max, Lag_max, Corr_min, Lag_min
    \end{lstlisting}
    }
    \end{minipage}
    \caption{Código de ejemplo en python.}
    \label{fig:originalCode}
    \end{figure*}

En la Figura~\ref{fig:originalCode} se muestra un ejemplo de uso de \verb+\lstlisting+ para insertar un bloque de código. En este ejemplo el código es Python, pero se puede cambiar el ``Syntax Highlighting'' cambiando el argumento \verb+language+, por ejemplo \verb+[language=C]+. Puedes hacer referencia a las líneas de código etiquetadas con \verb+(*@\label{lin:tu-etiqueta}@*)+, como por ejemplo las líneas~\ref{lin:xcm-a}-\ref{lin:xcm-b} del código.




